Restoring Incentive Compatibility in Two-Stage Energy Markets with Prosumers

A central challenge in modern energy market design is the formulation of a strategy-proof imbalance settlement layer that secures both the economic efficiency of the institution and the stability of the power grid. Public data reveals that the day-ahead market is strategically biased below actual consumer demand. Such empirical observations are explained by active prosumers which provide implementable incentives for demand under-reporting. Active prosumers buy energy in the day-ahead market and sell energy in the real-time market for balancing real-time energy deviations. By under-reporting their demand for the day ahead they inflate real-time imbalances and, under uniform pricing, they dispatch their generation assets more profitably. We model the two-stage institution under linear preferences and benchmark it against its associated competitive equilibria. We show that although consumers' incentives for demand under-reporting vanish when the day-ahead market scales, prosumers' incentives remain lower bounded by a positive gain which depends only on the real-time market generation stack and their shares over it. To restore incentive compatibility under the existing informational constraints, we design a leave-one-out contrastive scoring rule-based penalty that is implemented by the day-ahead market operator, incentivizes prosumers to report their demand truthfully and ensures small charges when participating honestly. We illustrate these results with numerical simulations on synthetic data and evaluate our mechanism on real-market data by first rationalizing demand reports as subjective equilibria of the induced game. Our mechanism demonstrates strong incentive alignment while retaining a low cost for honest participation.

==> styles.tex <==
\makeatletter
% Define a helper macro for uppercase letters (\mathrm{})
\def\autoMathrm#1{\ifmmode\mathrm{#1}\else#1\fi}
\def\rA{\autoMathrm{A}} \def\rB{\autoMathrm{B}} \def\rC{\autoMathrm{C}}
\def\rD{\autoMathrm{D}} \def\rE{\autoMathrm{E}} \def\rF{\autoMathrm{F}}
\def\rG{\autoMathrm{G}} \def\rH{\autoMathrm{H}} \def\rI{\autoMathrm{I}}
\def\rJ{\autoMathrm{J}} \def\rK{\autoMathrm{K}} \def\rL{\autoMathrm{L}}
\def\rM{\autoMathrm{M}} \def\rN{\autoMathrm{N}} \def\rO{\autoMathrm{O}}
\def\rP{\autoMathrm{P}} \def\rQ{\autoMathrm{Q}} \def\rR{\autoMathrm{R}}
\def\rS{\autoMathrm{S}} \def\rT{\autoMathrm{T}} \def\rU{\autoMathrm{U}}
\def\rV{\autoMathrm{V}} \def\rW{\autoMathrm{W}} \def\rX{\autoMathrm{X}}
\def\rY{\autoMathrm{Y}} \def\rZ{\autoMathrm{Z}}

% Define a helper macro for lowercase letters (\boldsymbol{})
\def\autoBoldsymbol#1{\ifmmode\boldsymbol{#1}\else#1\fi}
\def\a{\autoBoldsymbol{a}} \def\b{\autoBoldsymbol{b}} \def\c{\autoBoldsymbol{c}}
\def\d{\autoBoldsymbol{d}} \def\e{\autoBoldsymbol{e}} \def\f{\autoBoldsymbol{f}}
\def\g{\autoBoldsymbol{g}} \def\h{\autoBoldsymbol{h}} \def\i{\autoBoldsymbol{i}}
\def\j{\autoBoldsymbol{j}} \def\k{\autoBoldsymbol{k}} \def\l{\autoBoldsymbol{l}}
\def\m{\autoBoldsymbol{m}} \def\n{\autoBoldsymbol{n}} \def\o{\autoBoldsymbol{o}}
\def\p{\autoBoldsymbol{p}} \def\q{\autoBoldsymbol{q}} \def\r{\autoBoldsymbol{r}}
\def\s{\autoBoldsymbol{s}} \def\t{\autoBoldsymbol{t}} \def\u{\autoBoldsymbol{u}}
\def\v{\autoBoldsymbol{v}} \def\w{\autoBoldsymbol{w}} \def\x{\autoBoldsymbol{x}}
\def\y{\autoBoldsymbol{y}} \def\z{\autoBoldsymbol{z}}

% Define shortcuts for blackboard bold letters
\def\bA{\mathbb{A}} \def\bB{\mathbb{B}} \def\bC{\mathbb{C}} \def\bD{\mathbb{D}}
\def\bE{\mathbb{E}} \def\bF{\mathbb{F}} \def\bG{\mathbb{G}} \def\bH{\mathbb{H}}
\def\bI{\mathbb{I}} \def\bJ{\mathbb{J}} \def\bK{\mathbb{K}} \def\bL{\mathbb{L}}
\def\bM{\mathbb{M}} \def\bN{\mathbb{N}} \def\bO{\mathbb{O}} \def\bP{\mathbb{P}}
\def\bQ{\mathbb{Q}} \def\bR{\mathbb{R}} \def\bS{\mathbb{S}} \def\bT{\mathbb{T}}
\def\bU{\mathbb{U}} \def\bV{\mathbb{V}} \def\bW{\mathbb{W}} \def\bX{\mathbb{X}}
\def\bY{\mathbb{Y}} \def\bZ{\mathbb{Z}}

\def\rmd{\automathrm{d}}


% \fX for \mathfrak{X}, for all uppercase letters
\newcommand{\fA}{\mathfrak{A}} \newcommand{\fB}{\mathfrak{B}}
\newcommand{\fC}{\mathfrak{C}} \newcommand{\fD}{\mathfrak{D}}
\newcommand{\fE}{\mathfrak{E}} \newcommand{\fF}{\mathfrak{F}}
\newcommand{\fG}{\mathfrak{G}} \newcommand{\fH}{\mathfrak{H}}
\newcommand{\fI}{\mathfrak{I}} \newcommand{\fJ}{\mathfrak{J}}
\newcommand{\fK}{\mathfrak{K}} \newcommand{\fL}{\mathfrak{L}}
\newcommand{\fM}{\mathfrak{M}} \newcommand{\fN}{\mathfrak{N}}
\newcommand{\fO}{\mathfrak{O}} \newcommand{\fP}{\mathfrak{P}}
\newcommand{\fQ}{\mathfrak{Q}} \newcommand{\fR}{\mathfrak{R}}
\newcommand{\fS}{\mathfrak{S}} \newcommand{\fT}{\mathfrak{T}}
\newcommand{\fU}{\mathfrak{U}} \newcommand{\fV}{\mathfrak{V}}
\newcommand{\fW}{\mathfrak{W}} \newcommand{\fX}{\mathfrak{X}}
\newcommand{\fY}{\mathfrak{Y}} \newcommand{\fZ}{\mathfrak{Z}}

% \frx for \mathfrak{x}, for all lowercase letters
\newcommand{\fra}{\mathfrak{a}} \newcommand{\frb}{\mathfrak{b}}
\newcommand{\frc}{\mathfrak{c}} \newcommand{\frd}{\mathfrak{d}}
\newcommand{\fre}{\mathfrak{e}} \newcommand{\frf}{\mathfrak{f}}
\newcommand{\frg}{\mathfrak{g}} \newcommand{\frh}{\mathfrak{h}}
\newcommand{\fri}{\mathfrak{i}} \newcommand{\frj}{\mathfrak{j}}
\newcommand{\frk}{\mathfrak{k}} \newcommand{\frl}{\mathfrak{l}}
\newcommand{\frm}{\mathfrak{m}} \newcommand{\frn}{\mathfrak{n}}
\newcommand{\fro}{\mathfrak{o}} \newcommand{\frp}{\mathfrak{p}}
\newcommand{\frq}{\mathfrak{q}} \newcommand{\frr}{\mathfrak{r}}
\newcommand{\frs}{\mathfrak{s}} \newcommand{\frt}{\mathfrak{t}}
\newcommand{\fru}{\mathfrak{u}} \newcommand{\frv}{\mathfrak{v}}
\newcommand{\frw}{\mathfrak{w}} \newcommand{\frx}{\mathfrak{x}}
\newcommand{\fry}{\mathfrak{y}} \newcommand{\frz}{\mathfrak{z}}

\newcommand{\precc}{\underset{c}{\prec}}
\newcommand{\precceq}{\underset{c}{\preccurlyeq}}
\newcommand{\succv}{\underset{v}{\succ}}
\newcommand{\succc}{\underset{c}{\succ}}
\newcommand{\succveq}{\underset{v}{\succcurlyeq}}
\newcommand{\precv}{\underset{v}{\prec}}
\newcommand{\precveq}{\underset{v}{\preccurlyeq}}
\renewcommand{\k}{\kappa}



\newtheorem{example}{Example}
\newtheorem{question}{Question}
\newtheorem{problem}{Problem}
\newtheorem{theorem}{Theorem}
\newtheorem{assumption}{Assumption}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
